Estimating Extreme 3D Image Rotation with Transformer Cross-Attention

The estimation of large and extreme image rotation plays a key role in multiple computer vision domains, where the rotated images are related by a limited or a non-overlapping field of view. Contemporary approaches apply convolutional neural networks to compute a 4D correlation volume to estimate the relative rotation between image pairs. In this work, we propose a cross-attention-based approach that utilizes CNN feature maps and a Transformer-Encoder, to compute the cross-attention between the activation maps of the image pairs, which is shown to be an improved equivalent of the 4D correlation volume, used in previous works. In the suggested approach, higher attention scores are associated with image regions that encode visual cues of rotation. Our approach is end-to-end trainable and optimizes a simple regression loss. It is experimentally shown to outperform contemporary state-of-the-art schemes when applied to commonly used image rotation datasets and benchmarks, and establishes a new state-of-the-art accuracy on these datasets. We make our code publicly available.

==> figures/shay/results.tex <==
\begin{figure*}
\begin{minipage}{\linewidth}
    \begin{center}
    \newcommand{\sizea}{0.415\textwidth}
    \newcommand{\tal}{0cm}
    \newcommand{\tab}{0cm}
    \newcommand{\tar}{0cm}
    \newcommand{\tat}{0cm}
    \newcommand{\smb}{0cm}
    \newcommand{\T}[1]{\raisebox{-0.5\height}{#1}}
    \setlength{\tabcolsep}{0pt}
    \renewcommand{\arraystretch}{0}
    % \scriptsize
    \vspace{10pt}
    \begin{tabular} {cc} %{@{}cc@{}}
        % \multirow{2}{*}{\rotatebox[origin=l]{90}{Large \whitetxt{ss}}} &
        % \rotatebox[origin=l]{90}{Large } &
        \T{\includegraphics[width=\sizea, trim={\tal} {\tab} {\tar} {\tat},clip]{figure/shay/pan00.jpg}} &
        % \T{\includegraphics[width=0.2\textwidth, trim={\tal} {\tab} {\tar} {\tat},clip]{figure/shay/gt00_1.jpg}} &
        % \T{\includegraphics[width=0.2\textwidth, trim={\tal} {\tab} {\tar} {\tat},clip]{figure/shay/gt00_2.jpg}} &
        \T{\includegraphics[width=\sizea, trim={\tal} {\tab} {\tar} {\tat},clip]{figure/shay/panA06.jpg}} &
        % \T{\includegraphics[width=0.1\textwidth, trim={\tal} {\tab} {\tar} {\tat},clip]{figure/shay/gtA00_1.jpg}} &
        % \T{\includegraphics[width=0.1\textwidth, trim={\tal} {\tab} {\tar} {\tat},clip]{figure/shay/gtA00_2.jpg}}
        % \\  \vspace{+1pt}
        
        \T{\includegraphics[width=\sizea, trim={\tal} {\tab} {\tar} {\tat},clip]{figure/shay/pan01.jpg}} &
        % \T{\includegraphics[width=\sizea, trim={\tal} {\tab} {\tar} {\tat},clip]{figure/predicted_results/st_noalias/st_wo_img_pers_242_large.jpg}} &
        \T{\includegraphics[width=\sizea, trim={\tal} {\tab} {\tar} {\tat},clip]{figure/shay/panA07.jpg}}
        % \T{\includegraphics[width=\sizea, trim={\tal} {\tab} {\tar} {\tat},clip]{figure/predicted_results/sun360_noalias/sun360_img_pers_320_large.jpg}}
        \\ 
        % [+21pt]
        
        % \multirow{2}{*}{\rotatebox[origin=c]{90}{Small\whitetxt{ssss}}} &
        \T{\includegraphics[width=\sizea, trim={\tal} {\tab} {\tar} {\tat},clip]{figure/shay/pan02.jpg}} &
        % \T{\includegraphics[width=\sizea, trim={\tal} {\tab} {\tar} {\tat},clip]{figure/predicted_results/st_noalias/st_wo_img_pers_703_small.jpg}} &
        \T{\includegraphics[width=\sizea, trim={\tal} {\tab} {\tar} {\tat},clip]{figure/shay/panA02.jpg}} &
        % \T{\includegraphics[width=\sizea, trim={\tal} {\tab} {\tar} {\tat},clip]{figure/predicted_results/sun360_noalias/sun360_img_pers_21_small.jpg}}
        % \\ \vspace{+1pt}
        % [+21pt]
        
        % \T{\includegraphics[width=\sizea, trim={\tal} {\tab} {\tar} {\tat},clip]{figure/predicted_results/st_noalias/st_wo_img_pano_36_small.jpg}} &
        \T{\includegraphics[width=\sizea, trim={\tal} {\tab} {\tar} {\tat},clip]{figure/shay/pan03.jpg}} &
        \T{\includegraphics[width=\sizea, trim={\tal} {\tab} {\tar} {\tat},clip]{figure/shay/panA03.jpg}} &
        % \T{\includegraphics[width=\sizea, trim={\tal} {\tab} {\tar} {\tat},clip]{figure/predicted_results/sun360_noalias/sun360_img_pers_291_small.jpg}}
        \\
        % \multirow{2}{*}{\rotatebox[origin=c]{90}{None\whitetxt{sssss}}} &
        % \T{\includegraphics[width=\sizea, trim={\tal} {\tab} {\tar} {\tat},clip]{figure/predicted_results/st_noalias/st_wo_img_pano_105_non.jpg}} &
        \T{\includegraphics[width=\sizea, trim={\tal} {\tab} {\tar} {\tat},clip]{figure/shay/pan04.jpg}} &
        \T{\includegraphics[width=\sizea, trim={\tal} {\tab} {\tar} {\tat},clip]{figure/shay/panA04.jpg}} &
        % \T{\includegraphics[width=\sizea, trim={\tal} {\tab} {\tar} {\tat},clip]{figure/predicted_results/sun360_noalias/sun360_img_pers_46_non.jpg}}
        % \\  \vspace{+2pt}
        % [+21pt]
        
        % \T{\includegraphics[width=\sizea, trim={\tal} {\tab} {\tar} {\tat},clip]{figure/predicted_results/st_noalias/st_wo_img_pano_11_non.jpg}} &
        \T{\includegraphics[width=\sizea, trim={\tal} {\tab} {\tar} {\tat},clip]{figure/shay/pan05.jpg}} &
        \T{\includegraphics[width=\sizea, trim={\tal} {\tab} {\tar} {\tat},clip]{figure/shay/panA05.jpg}} 
        % \T{\includegraphics[width=\sizea, trim={\tal} {\tab} {\tar} {\tat},clip]{figure/predicted_results/sun360_noalias/sun360_img_pers_67_non.jpg}}
        % \\ \vspace{-2pt}
        % & \multicolumn{2}{r}{StreetLearn} 
        % & StreetLearn W/ Trans. 
        % & \multicolumn{2}{l}{SUN360} 
    \end{tabular}
\vspace{-10pt}
    \end{center}
    \caption{\textbf{Predicted rotation results.} Full panoramas are shown with their cropped ground-truth perspective images marked in green. Our predicted viewpoints results are shown with a dot-yellow line the first viewpoint (fixed) and with dot-red line the second predicted viewpoints which determined by the relative angle predicted values i.e. Yaw and Tilt. The overlapping fractions are ordered as follows: the first two rows introduce a large-overlapping, the next two rows introduce a small-overlapping and the last two rows introduced none-overlapping.
    }
    \label{fig:predicted}
\end{minipage}
\end{figure*}



% \begin{figure*}
% \begin{minipage}{\linewidth}
%     \begin{center}
%     \newcommand{\sizea}{0.235\textwidth}
%     \newcommand{\tal}{0cm}
%     \newcommand{\tab}{0cm}
%     \newcommand{\tar}{0cm}
%     \newcommand{\tat}{0cm}
%     \newcommand{\smb}{0cm}
%     \newcommand{\T}[1]{\raisebox{-0.5\height}{#1}}
%     \setlength{\tabcolsep}{0pt}
%     \renewcommand{\arraystretch}{0}
%     % \scriptsize
%     \vspace{10pt}
%     \begin{tabular}{@{}ccccc@{}}
%         \multirow{2}{*}{\rotatebox[origin=c]{90}{Large \whitetxt{ssss}}} &
%         \T{\includegraphics[width=\sizea, trim={\tal} {\tab} {\tar} {\tat},clip]{figure/predicted_results/st_noalias/st_wo_img_pano_22_large.jpg}} &
%         \T{\includegraphics[width=\sizea, trim={\tal} {\tab} {\tar} {\tat},clip]{figure/predicted_results/st_noalias/st_wo_img_pers_22_large.jpg}} &
%         \T{\includegraphics[width=\sizea, trim={\tal} {\tab} {\tar} {\tat},clip]{figure/predicted_results/sun360_noalias/sun360_img_pano60_large.jpg}}&
%         \T{\includegraphics[width=\sizea, trim={\tal} {\tab} {\tar} {\tat},clip]{figure/predicted_results/sun360_noalias/sun360_img_pers_60_large.jpg}}
%         \\  \vspace{+1pt}
%         &

==> table/comb_ablation_table.tex <==
\begin{table}[]
\centering
\scriptsize
\setlength{\tabcolsep}{1.0pt}
\resizebox{\columnwidth}{!}{
\begin{tabular}{llccclcclcc} 
\toprule
\multicolumn{2}{l}{}                         & \multicolumn{3}{c}{Rotation Error}&  & \multicolumn{2}{c}{Yaw Error}                                                                       &  & \multicolumn{2}{c}{Pitch Error}\\  \cline{3-5} \cline{7-8} \cline{10-11}
Overlap & Method
& Avg(\degree) & Med(\degree) & \multicolumn{1}{c}{10\degree(\%)} & & Avg(\degree) & Med(\degree) & & Avg(\degree) & Med(\degree)
\\ \midrule
\multirow{5}{*}{Large} & w/o RP                              & 1.02         & 1.05         & 100.00 &  & 0.48          & 0.47          &  & 0.52           & 0.48           \\
                       & w/o $\mathcal{L}_\mathsf{cls},\mathcal{C}$ & 40.19        & 33.41        & 8.87   &  & 33.22         & 23.19         &  & 16.50          & 14.01          \\
                       & w/o $\mathcal{L}_\mathsf{cls}$             & 7.93         & 6.96         & 78.33  &  & 5.07          & 3.90          &  & 3.22           & 2.91           \\
                       & w/o $\mathcal{C}$                   & 43.79        & 43.44        & 6.90   &  & 43.74         & 43.44         &  & 1.07           & 0.74           \\
                       & Ours (full)                         & 1.37         & 1.09         & 99.51  &  & 0.57          & 0.51          &  & 1.03           & 0.73           \\ \midrule
\multirow{5}{*}{Small} & w/o RP                              & 1.67         & 1.44         & 99.62  &  & 0.83          & 0.61          &  & 0.79           & 0.64           \\
                       & w/o $\mathcal{L}_\mathsf{cls},\mathcal{C}$ & 67.97        & 60.91        & 0.38   &  & 61.53         & 54.19         &  & 19.71          & 15.59          \\
                       & w/o $\mathcal{L}_\mathsf{cls}$             & 15.75        & 12.65        & 34.59  &  & 10.28         & 6.35          &  & 5.81           & 4.31           \\
                       & w/o $\mathcal{C}$                   & 65.31        & 69.32        & 15.79  &  & 65.13         & 69.31         &  & 2.04           & 1.10           \\
                       & Ours (full)                         & 6.13         & 1.77         & 95.86  &  & 4.70          & 0.72          &  & 1.76           & 0.97           \\ \midrule
\multirow{5}{*}{None}  & w/o RP                              & 39.01        & 25.81        & 23.92  &  & 36.32         & 21.17         &  & 5.96           & 3.39           \\
                       & w/o $\mathcal{L}_\mathsf{cls},\mathcal{C}$ & 83.29        & 75.08        & 0.56   &  & 78.42         & 68.89         &  & 18.16          & 14.72          \\
                       & w/o $\mathcal{L}_\mathsf{cls}$             & 46.26        & 39.53        & 2.64   &  & 40.98         & 34.08         &  & 13.93          & 11.08          \\
                       & w/o $\mathcal{C}$                   & 121.16       & 130.91       & 0.19   &  & 121.10        & 130.91        &  & 1.97           & 1.26           \\
                       & Ours (full)                         & 34.92        & 4.43         & 61.39  &  & 34.19         & 3.51          &  & 1.91           & 1.36           \\ \midrule
\multirow{5}{*}{All}   & w/o RP                              & 21.37        & 3.98         & 59.50  &  & 19.60         & 1.87          &  & 3.48           & 1.09           \\
                       & w/o $\mathcal{L}_\mathsf{cls},\mathcal{C}$ & 70.46        & 57.87        & 2.20   &  & 64.75         & 52.70         &  & 18.24          & 14.72          \\
                       & w/o $\mathcal{L}_\mathsf{cls}$             & 30.36        & 19.97        & 26.50  &  & 25.52         & 12.61         &  & 9.60           & 5.88           \\
                       & w/o $\mathcal{C}$                   & 90.60        & 89.37        & 5.70   &  & 90.51         & 89.35         &  & 1.81           & 1.10           \\
                       & Ours (full)                         & 20.45        & 2.23         & 78.30  &  & 19.52         & 1.07          &  & 1.69           & 1.07          
                       \\ \bottomrule              
\end{tabular}%
}
\vspace{-8pt}
\caption{\textbf{Ablation study},
evaluating the effect of our rotation parameterization (RP), classification objective ($\mathcal{L}_\mathsf{cls}$) and correlation volumes ($\mathcal{C}$) on SUN360.
}
\label{tab:ablation}
\end{table}




==> table/final_main_table_correct.tex <==
\definecolor{graytext}{RGB}{130,130,130}

\begin{table*}[t]
\setlength{\tabcolsep}{1.0pt}
% \def\arraystretch{1.05}
 \def\arraystretch{0.95}
%  \footnotesize
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccclccclccclccclccc}
\toprule
\multicolumn{2}{l}{}& \multicolumn{3}{c}{InteriorNet} &  & \multicolumn{3}{c}{InteriorNet-T} &  & \multicolumn{3}{c}{SUN360} &  & \multicolumn{3}{c}{StreetLearn} &  & \multicolumn{3}{c}{StreetLearn-T}\\ \cline{3-5} \cline{7-9} \cline{11-13} \cline{15-17} \cline{19-21}
Overlap 
& Method
& Avg(\degree$\downarrow$) & Med(\degree$\downarrow$) & \multicolumn{1}{c}{10\degree(\%$\uparrow$)} & & Avg(\degree$\downarrow$) & Med(\degree$\downarrow$) & \multicolumn{1}{c}{10\degree(\%$\uparrow$)} &  & Avg(\degree$\downarrow$) & Med(\degree$\downarrow$) & \multicolumn{1}{c}{10\degree(\%$\uparrow$)} &  & Avg(\degree$\downarrow$) & Med(\degree$\downarrow$) & \multicolumn{1}{c}{10\degree(\%$\uparrow$)} &  & Avg(\degree$\downarrow$) & Med(\degree$\downarrow$) & \multicolumn{1}{c}{10\degree(\%$\uparrow$)} \\ \midrule
\multirow{6}{*}{Large} & SIFT*~\cite{lowe2004distinctive}       & 6.09                 & 4.00                 & 84.86               &  & 7.78                 & 2.95                 & 55.52               &  & 5.46                       & 3.88                       & 93.10                      &  & 5.84                 & 3.16                 & 91.18               &  & \color{graytext}{18.86}                & \color{graytext}{3.13}                 & \color{graytext}{22.37}               \\
                        %  & SuperPoint*~\cite{detone18superpoint}  & 5.40                 & 3.53                 & 87.10               &  & 5.46                 & 2.79                 & 65.97               &  & 4.69                       & 3.18                       & 92.12                      &  & 6.23                 & 3.61                 & 91.18               &  & \textbf{6.38}        & \textbf{1.79}        & 16.45               \\
                         & SuperPoint*~\cite{detone18superpoint}  & 5.40                 & 3.53                 & 87.10               &  & 5.46                 & 2.79                 & 65.97               &  & 4.69                       & 3.18                       & 92.12                      &  & 6.23                 & 3.61                 & 91.18               &  & \color{graytext}{6.38}        & \color{graytext}{1.79}        & \color{graytext}{16.45}               \\
                         & Reg6D~\cite{zhou2019continuity}-o     & 5.43                 & 3.87                 & 87.10               &  & 10.45                & 6.91                 & 67.76               &  & 7.18                       & 5.79                       & 81.28                      &  & 3.36                 & 2.71                 & 97.65               &  & 12.31                & 6.02                 & 69.08               \\
                         & Reg6D~\cite{zhou2019continuity}        & 9.05                 & 5.90                 & 68.49               &  & 17.00                & 11.95                & 41.79               &  & 16.51                      & 12.43                      & 40.39                      &  & 11.70                & 8.87                 & 58.24               &  & 36.71                & 24.79                & 23.03               \\
                         & Ours-o                                & \textbf{1.53}        & 1.10                 & \textbf{99.26}     &  & \textbf{2.89}        & \textbf{1.10}        & \textbf{97.61}     &  & \textbf{1.00}              & \textbf{0.94}              & \textbf{100.00}           &  & \textbf{1.19}        & \textbf{1.02}        & \textbf{99.41}     &  & \textbf{9.12}                 & 2.91                 & \textbf{87.50}     \\
                        %  & Ours                                   & 1.82                 & \textbf{0.88}        & 98.76               &  & 8.86                 & 1.86                 & 93.13               &  & 1.37                       & 1.09                       & 99.51                      &  & 1.52                 & 1.09                 & \textbf{99.41}     &  & 24.98                & 2.48                 & 78.95               \\ \cline{2-21}
                         & Ours                                   & 1.82                 & \textbf{0.88}        & 98.76               &  & 8.86                 & 1.86                 & 93.13               &  & 1.37                       & 1.09                       & 99.51                      &  & 1.52                 & 1.09                 & \textbf{99.41}     &  & 24.98                & \textbf{2.48}                 & 78.95               \\ \midrule%\cline{2-21}
                        % & Training                               & 0.77          & 0.71          & 99.73          &  & 2.15           & 1.36          & 98.71          &  & 0.81          & 0.80          & 100.00          &  & 1.03          & 0.92          & 99.96          &  & 3.49          & 1.28          & 96.91          \\ \midrule
\multirow{6}{*}{Small} & SIFT*~\cite{lowe2004distinctive}       & 24.18                & 8.57                 & 39.73               &  & \color{graytext}{18.16}                & \color{graytext}{10.01}                & \color{graytext}{18.52}               &  & 13.71                      & 6.33                       & 56.77                      &  & 16.22                & 7.35                 & 55.81               &  & \color{graytext}{38.78}                & \color{graytext}{13.81}                & \color{graytext}{5.68}                \\
                         & SuperPoint*~\cite{detone18superpoint}  & \color{graytext}{16.72}                & \color{graytext}{8.43}                 & \color{graytext}{21.58}               &  & \color{graytext}{11.61}                & \color{graytext}{5.82}                 & \color{graytext}{11.73}               &  & \color{graytext}{17.63}                      & \color{graytext}{7.70}                       & \color{graytext}{26.69}                      &  & \color{graytext}{19.29}                & \color{graytext}{7.60}                 & \color{graytext}{24.58}               &  & \color{graytext}{6.80}        & \color{graytext}{6.85}                 & \color{graytext}{0.95}                \\
                         & Reg6D~\cite{zhou2019continuity}-o     & 17.83                & 9.61                 & 51.37               &  & 21.87                & 11.43                & 44.14               &  & 18.61                      & 11.66                      & 39.85                      &  & 7.95                 & 4.34                 & 87.71               &  & 15.07                & 7.59                 & 63.41               \\
                         & Reg6D~\cite{zhou2019continuity}        & 25.71                & 15.56                & 33.56               &  & 42.93                & 28.92                & 23.15               &  & 42.55                      & 32.11                      & 9.40                       &  & 24.77                & 15.11                & 30.56               &  & 46.61                & 34.33                & 13.88               \\
                         & Ours-o                                & 6.45                 & 1.61                 & 95.89               &  & \textbf{10.24}       & \textbf{1.38}        & \textbf{89.81}     &  & \textbf{3.09}              & \textbf{1.41}              & \textbf{98.50}            &  & \textbf{2.32}        & \textbf{1.41}        & \textbf{98.67}     &  & \textbf{13.04}                & 3.49                 & \textbf{84.23}     \\
                         & Ours                                   & \textbf{4.31}        & \textbf{1.16}        & \textbf{96.58}     &  & 30.43                & 2.63                 & 74.07               &  & 6.13                       & 1.77                       & 95.86                      &  & 3.23                 & \textbf{1.41}        & 98.34               &  & 27.84                & \textbf{3.19}        & 74.76               \\ \midrule%\cline{2-21}
                        % & Training                               & 3.57          & 0.88          & 98.34          &  & 9.13           & 1.47          & 94.75          &  & 1.81          & 1.03          & 99.26           &  & 1.46          & 1.13          & 99.80          &  & 4.23          & 1.44          & 96.22          \\ \midrule
\multirow{5}{*}{None}   & SIFT*~\cite{lowe2004distinctive}       & \color{graytext}{109.30}               & \color{graytext}{92.86}                & \color{graytext}{0.00}                &  & \color{graytext}{93.79}                & \color{graytext}{113.86}               & \color{graytext}{0.00}                &  & \color{graytext}{127.61}                     & \color{graytext}{129.07}                     & \color{graytext}{0.00}                       &  & \color{graytext}{83.49}                & \color{graytext}{90.00}                & \color{graytext}{0.38}                &  & \color{graytext}{85.90}                & \color{graytext}{106.84}               & \color{graytext}{0.38}                \\
                         & SuperPoint*~\cite{detone18superpoint}  & \color{graytext}{120.28}               & \color{graytext}{120.28}               & \color{graytext}{0.00}                &  & \color{graytext}{--}                   & \color{graytext}{--}                   & \color{graytext}{0.00}                &  & \color{graytext}{149.80}                     & \color{graytext}{165.24}                     & \color{graytext}{0.00}                       &  & \color{graytext}{--}                   & \color{graytext}{--}                   & \color{graytext}{0.00}                &  & \color{graytext}{--}                   & \color{graytext}{--}                   & \color{graytext}{0.00}                \\
                          & Reg6D~\cite{zhou2019continuity}-o  & 88.89                            & 79.24                            & 0.98                         &  & 110.50                           & 116.25                           & 1.17                         &  & 101.21                           & 99.64                            & 0.94                         &  & 133.08       & 167.19       & 2.46     &  & 132.67       & 158.45       & 1.88     \\
                         & Reg6D~\cite{zhou2019continuity}        & 48.36                & 32.93                & 10.82               &  & 60.91                & 51.26                & 11.14               &  & 64.74                      & 56.55                      & 3.77                       &  & 28.48                & 18.86                & 24.39               &  & 49.23                & 35.66                & 11.86               \\
                         & Ours                                   & \textbf{37.69}       & \textbf{3.15}        & \textbf{61.97}     &  & \textbf{49.44}       & \textbf{4.17}        & \textbf{58.36}     &  & \textbf{34.92}             & \textbf{4.43}              & \textbf{61.39}            &  & \textbf{5.77}        & \textbf{1.53}        & \textbf{96.41}     &  & \textbf{30.98}       & \textbf{3.50}        & \textbf{72.69}     \\ \midrule%\cline{2-21}
                        % & Training                               & 26.16         & 1.41          & 73.21          &  & 19.71          & 2.04          & 84.97          &  & 27.18         & 2.02          & 69.51           &  & 3.18          & 1.36          & 98.62          &  & 18.41         & 1.94          & 83.50          \\ \midrule
\multirow{5}{*}{All}    & SIFT*~\cite{lowe2004distinctive}       & 13.68                & 5.04                 & 45.80               &  & \color{graytext}{12.24}                & \color{graytext}{5.69}                 & \color{graytext}{24.60}               &  & \color{graytext}{18.12}                      & \color{graytext}{5.02}                       & \color{graytext}{34.00}                      &  & \color{graytext}{17.29}                & \color{graytext}{5.53}                 & \color{graytext}{32.50}               &  & \color{graytext}{36.00}                & \color{graytext}{6.03}                 & \color{graytext}{5.40}                \\
                         %& SuperPoint*~\cite{detone18superpoint}  & \textbf{8.19}        & 4.08                 & 41.40               &  & \textbf{6.62}        & 3.38                 & 25.90               &  & \textbf{11.09}             & 4.00                       & 25.80                      &  & 11.52                & 4.80                 & 22.90               &  & \color{graytext}{6.42}        & \color{graytext}{2.62}        & 2.80                \\
                         & SuperPoint*~\cite{detone18superpoint}  & \color{graytext}{8.19}        & \color{graytext}{4.08}                 & \color{graytext}{41.40}               &  & \color{graytext}{6.62}        & \color{graytext}{3.38}                 & \color{graytext}{25.90}               &  & \color{graytext}{11.09}             & \color{graytext}{4.00}                       & \color{graytext}{25.80}                      &  & \color{graytext}{11.52}                & \color{graytext}{4.80}                 & \color{graytext}{22.90}               &  & \color{graytext}{6.42}        & \color{graytext}{2.62}        & \color{graytext}{2.80}                \\
                          & Reg6D~\cite{zhou2019continuity}-o     & 34.51                            & 9.71                             & 50.40                        &  & 48.27                            & 15.59                            & 37.40                        &  & 60.15                            & 34.51                            & 27.60                        &  & 73.36        & 20.03        & 44.30    &  & 77.09        & 55.29        & 31.60\\ 
                         & Reg6D~\cite{zhou2019continuity}        & 25.90                & 13.02                & 40.70               &  & 40.38                & 23.35                & 25.30               &  & 49.05                      & 34.37                      & 12.70                      &  & 24.51                & 15.31                & 32.00               &  & 46.50                & 33.14                & 29.90               \\
                         & Ours                                   & \textbf{13.49}                & \textbf{1.18}        & \textbf{86.90}     &  & \textbf{29.68}                & \textbf{2.58}        & \textbf{75.10}     &  & \textbf{20.45}                      & \textbf{2.23}              & \textbf{78.30}            &  & \textbf{4.40}        & \textbf{1.44}        & \textbf{97.50}     &  & \textbf{29.85}                & \textbf{3.20}                 & \textbf{74.30}     \\ %\cline{2-21}
                        % & Training                               & 9.77          & 0.91          & 90.80          &  & 10.84          & 1.60          & 92.40          &  & 14.66         & 1.25          & 84.10           &  & 2.58          & 1.19          & 98.96          &  & 15.90         & 1.78          & 85.79         \\
                        \bottomrule 
\end{tabular}
}
\vspace{-8pt}
\caption{\textbf{Rotation estimation evaluation on the InteriorNet, the SUN360, and the StreetLearn datasets.} 
We report the mean and median geodesic error in degrees, and the percentage of pairs with a relative rotation error under 10$\degree$ for different levels of overlap, as detailed in Section \ref{sec:metrics}. %For the percentage of pairs (10$\degree$\%), higher is better. 
Models trained only on overlapping pairs are denoted with ``-o''.
% We report the mean and median geodesic error in degrees, and the percentage of pairs with a relative rotation error under 10$\degree$, for different levels (Small, Medium, and Large), as detailed in Section 4.3 of the main paper. For the percentage of pairs (10$\degree$\%), higher is better. Models trained only on overlapping pairs are denoted with ``-o''.
* indicates mean/median errors are computed only over successful image pairs, for which these algorithms output a pose estimate (failure over more than $50\%$ of the test pairs is shown in gray).}
\label{tab:main_result}
\end{table*}

==> table/final_pair.tex <==
\begin{table*}[]
\setlength{\tabcolsep}{2.3pt}
% \def\arraystretch{1.05}
\small
\begin{center}
\begin{tabularx}{\textwidth}{llcccccccccccccccccccc}
\toprule

 & &\multicolumn{3}{c}{InteriorNet}   &  & \multicolumn{3}{c}{InteriorNet-T} &  & \multicolumn{3}{c}{SUN360} &  & \multicolumn{3}{c}{StreetLearn}  &  & \multicolumn{3}{c}{StreetLearn-T} \\  \cline{3-5} \cline{7-9} \cline{11-13} \cline{15-17} \cline{19-21}
\%Overlap & Method     & Success & Fail & Total & & Success & Fail & Total & & Success & Fail & Total &  & Success & Fail & Total &  & Success & Fail & Total \\ \midrule
\multirow{3}{*}{Large} & SIFT~\cite{lowe2004distinctive}      & 371 & 32  & 403  &  & 252 & 83  & 335  &  & 201 & 2   & 203  &  & 166 & 4   & 170  &  & 50  & 102 & 152  \\
                       & D2-Net~\cite{Dusmanu2019CVPR}        & 330 & 73  & 403  &  & 102 & 233 & 335  &  & 176 & 27  & 203  &  & 119 & 51  & 170  &  & 3   & 149 & 152  \\
                       & SuperPoint~\cite{detone18superpoint} & 382 & 21  & 403  &  & 259 & 76  & 335  &  & 201 & 2   & 203  &  & 169 & 1   & 170  &  & 30  & 122 & 152  \\ \midrule
\multirow{3}{*}{Small} & SIFT~\cite{lowe2004distinctive}      & 195 & 97  & 292  &  & 121 & 203 & 324  &  & 217 & 49  & 266  &  & 267 & 34  & 301  &  & 39  & 278 & 317  \\
                       & D2-Net~\cite{Dusmanu2019CVPR}        & 17  & 275 & 292  &  & 0   & 324 & 324  &  & 23  & 243 & 266  &  & 17  & 284 & 301  &  & 1   & 316 & 317  \\
                       & SuperPoint~\cite{detone18superpoint} & 112 & 180 & 292  &  & 60  & 264 & 324  &  & 112 & 154 & 266  &  & 115 & 186 & 301  &  & 3   & 314 & 317  \\ \midrule
\multirow{3}{*}{None}  & SIFT~\cite{lowe2004distinctive}      & 8   & 297 & 305  &  & 5   & 336 & 341  &  & 32  & 499 & 531  &  & 27  & 502 & 529  &  & 15  & 516 & 531  \\
                       & D2-Net~\cite{Dusmanu2019CVPR}        & 0   & 305 & 305  &  & 0   & 341 & 341  &  & 2   & 529 & 531  &  & 0   & 529 & 529  &  & 0   & 531 & 531  \\
                       & SuperPoint~\cite{detone18superpoint} & 1   & 304 & 305  &  & 0   & 341 & 341  &  & 4   & 527 & 531  &  & 0   & 529 & 529  &  & 0   & 531 & 531  \\ \midrule
\multirow{3}{*}{All}   & SIFT~\cite{lowe2004distinctive}      & 574 & 426 & 1000 &  & 378 & 622 & 1000 &  & 450 & 550 & 1000 &  & 460 & 540 & 1000 &  & 104 & 896 & 1000 \\
                       & D2-Net~\cite{Dusmanu2019CVPR}        & 347 & 653 & 1000 &  & 102 & 898 & 1000 &  & 201 & 799 & 1000 &  & 136 & 864 & 1000 &  & 4   & 996 & 1000 \\
                       & SuperPoint~\cite{detone18superpoint} & 495 & 505 & 1000 &  & 319 & 681 & 1000 &  & 317 & 683 & 1000 &  & 284 & 716 & 1000 &  & 33  & 967 & 1000 \\
                        \bottomrule 
\end{tabularx}%
\end{center}
\vspace{-5pt}
\caption{\textbf{Number of pairs for which SIFT, D2-Net, and SuperPoint return an answer. }  For each dataset and overlap ratio, we report the number of pairs for which RANSAC successfully outputs a model (regardless of whether that model is accurate or not).
%*Note that SIFT fails to output a homography for some image pairs. We disregard these for the mean and median error computation.
}
\label{tab:sift_result}
\end{table*}

==> table/final_roll.tex <==
\begin{table*}[]
\centering
%  \footnotesize
%  \small
\setlength{\tabcolsep}{3.5pt}
%\def\arraystretch{1.15}
\begin{tabularx}{0.92\textwidth}{llccclccclccc} %0.91
%  \begin{tabularx}{0.91\textwidth}{llccllccllccll}
\toprule
\multicolumn{2}{l}{}                         & \multicolumn{3}{c}{Rotation Error}                                                                     &  & \multicolumn{3}{c}{Yaw Error}                                                                       &  & \multicolumn{3}{c}{Pitch Error}                                                                                  \\ \cline{3-5} \cline{7-9} \cline{11-13}
%\multicolumn{2}{l}{}        
\%Overlap & Roll
& Avg(\degree$\downarrow$) & Med(\degree$\downarrow$) & \multicolumn{1}{c}{10\degree(\%$\uparrow$)} &  & Avg(\degree$\downarrow$) & Med(\degree$\downarrow$) & \multicolumn{1}{c}{10\degree(\%$\uparrow$)} &  & Avg(\degree$\downarrow$) & Med(\degree$\downarrow$) & \multicolumn{1}{c}{10\degree(\%$\uparrow$)}  %\multicolumn{1}{c}{3\degree(\%$$\uparrow$)}  
\\ \midrule
\multirow{2}{*}{Large}                        & $=0\degree$  & 2.27 & 1.07 & 99.41 &  & 1.86 & 0.67 & 99.41 &  & 0.70 & 0.53 & 100.00 \\
 & $<5\degree$ & 7.71 & 3.18 & 97.08 &  & 5.20 & 0.84 & 97.65 &  & 1.55 & 1.55 & 99.41  \\ \midrule
\multirow{2}{*}{Small}                        & $=0\degree$  & 2.66 & 1.41 & 98.34 &  & 2.12 & 0.87 & 98.67 &  & 0.87 & 0.61 & 99.67  \\
 & $<5\degree$ & 6.43 & 3.39 & 96.33 &  & 3.43 & 0.95 & 98.01 &  & 1.56 & 0.87 & 99.00  \\\midrule
\multirow{2}{*}{None}                        & $=0\degree$  & 6.48 & 1.58 & 96.60 &  & 5.70 & 0.92 & 96.79 &  & 1.18 & 0.59 & 99.24  \\
  & $<5\degree$ & 8.54 & 3.44 & 96.22 &  & 6.88 & 1.16 & 96.22 &  & 1.37 & 0.87 & 99.24  \\\midrule
\multirow{2}{*}{All}                        & $=0\degree$  & 4.61 & 1.42 & 97.60 &  & 3.97 & 0.85 & 97.80 &  & 1.00 & 0.59 & 99.50  \\
   & $<5\degree$ & 7.77 & 3.39 & 96.40 &  & 5.56 & 1.04 & 97.00 &  & 1.46 & 0.88 & 99.20 \\
                        \bottomrule              
\end{tabularx}%

\caption{\textbf{Roll angle experiments on StreetLearn}, evaluating the effect of adding small roll angles to the ground truth rotation on relative rotation estimates of image pairs at test time. As illustrated in the table, adding roll at test time does not break the model, but rather leads to a modest increase in up to $2\degree$ error (across all overlap levels).
}
\label{tab:roll_supp}
\end{table*}

==> table/final_watermark.tex <==
\begin{table}[]
\centering
% \small
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabularx}{0.92\columnwidth}{llccclccc} 
\toprule
 & \multicolumn{3}{c}{w/ Watermarks}                                                                     &  & \multicolumn{3}{c}{w/o Watermarks}                                                                                                                                                       \\ \cline{2-4} \cline{6-8}
\%Overlap
& Avg(\degree$\downarrow$) & Med(\degree$\downarrow$) & \multicolumn{1}{c}{10\degree(\%$\uparrow$)} &  & Avg(\degree$\downarrow$) & Med(\degree$\downarrow$) & \multicolumn{1}{c}{10\degree(\%$\uparrow$)} 
\\ \midrule
Large & 1.52         & 1.09         & 99.41    &  & 3.52         & 1.13         & 98.24    \\
Small & 3.23         & 1.41         & 98.34    &  & 4.65         & 1.54         & 97.67    \\
None  & 5.77         & 1.53         & 96.41    &  & 9.18         & 1.81         & 94.33   \\
All   & 4.40         & 1.44         & 97.50    &  & 6.86         & 1.59         & 96.00   \\
                        \bottomrule              
\end{tabularx}%
\vspace{-5pt}
\caption{\textbf{Watermark removal experiment on StreetLearn}, showing results on the original test set on the left (w/ Watermarks) and on the modified test set on the right (w/o Watermarks). %As shown above, the median errors are almost the same in both cases, while average errors slightly increase after watermarks are removed from the test panoramas. 
% This experiment further illustrates that our StreetLearn model also reasons about \rrev{additional implicit cues besides the watermarks. }
This experiment further demonstrates that our model is not merely learning from spurious features like watermarks, but is leveraging a broader range of cues.
}
\label{tab:watermark_supp}
\end{table}

%       & \multicolumn{3}{c}{W/ Watermark}        &  & \multicolumn{3}{c}{W/O Watermark}       \\
%       & Avg(\degree) & Med(\degree) & 10\degree &  & Avg(\degree) & Med(\degree) & 10\degree \\
% Large & 1.52         & 1.09         & 99.41%    &  & 3.52         & 1.13         & 98.24%    \\
% Small & 3.23         & 1.41         & 98.34%    &  & 4.65         & 1.54         & 97.67%    \\
% None  & 5.77         & 1.53         & 96.41%    &  & 9.18         & 1.81         & 94.33%    \\
% All   & 4.40         & 1.44         & 97.50%    &  & 6.86         & 1.59         & 96.00%   
